Syntactic Inductive Biases for Deep Learning Methods

In this thesis, we try to build a connection between the two schools by introducing syntactic inductive biases for deep learning models. We propose two families of inductive biases, one for constituency structure and another one for dependency structure. The constituency inductive bias encourages deep learning models to use different units (or neurons) to separately process long-term and short-term information. This separation provides a way for deep learning models to build the latent hierarchical representations from sequential inputs, that a higher-level representation is composed of and can be decomposed into a series of lower-level representations. For example, without knowing the ground-truth structure, our proposed model learns to process logical expression through composing representations of variables and operators into representations of expressions according to its syntactic structure. On the other hand, the dependency inductive bias encourages models to find the latent relations between entities in the input sequence. For natural language, the latent relations are usually modeled as a directed dependency graph, where a word has exactly one parent node and zero or several children nodes. After applying this constraint to a Transformer-like model, we find the model is capable of inducing directed graphs that are close to human expert annotations, and it also outperforms the standard transformer model on different tasks. We believe that these experimental results demonstrate an interesting alternative for the future development of deep learning models.

==> sec_future.tex <==
\chapter{The Future of Syntactic Inductive Bias} \label{cha:future}

In previous chapters, we have described several models developed from different syntactic inductive biases. 
They provide some useful new feature or functionalities.
However these progress are just first few steps towards some long-term goals of the field.
In this chapter, we will discuss some important milestones for the future of syntactic inductive biases. 
We first review the current state of the unsupervised parsing and envisage the future of this task.
We then discuss how syntactic functions, another important component of syntax, can be revived in the context of deep learning.
Finally, we will discuss about one of the most important practical goals of syntactic inductive bias -- increasing the systematic generalization ability of deep learning models.

\section{Emerging Discrete Structure}
Syntactic inductive biases are first proposed as a guideline to develop unsupervised parsing models.
For most of the current methods, the induced structure is greedy sampled from a distribution of all possible structures.
Almost all methods focus on evaluating the coherence between the sampled structure and the gold structure given by expert annotators. 
The sharpness for the distribution is usually not taken into consideration.
However, as we argued in the introduction, the other important role of syntactic inductive bias is to regularize the internal connection of neural network models.
In this case a smooth distribution could result in a weak or non regularization effect.
For example, in UDGN, if the dependency distribution is uniform distribution for all words, then the latent structure of the model reduces to a fully connected.
In Ordered Memory, if the attention distribution at every time step is a uniform distribution, the model cannot compose information as a recursive neural network and lose its generalization ability.
Similarly, in Option-Controller Network, learning reusable skills also require the structural decisions to be sharp.
Hence, we would like to argue that the sharpness of distribution is at least as important as the correctness of induced latent structure for tasks that require strong generalization ability.

On the other hand, encourage a sharp distribution is also an important step towards combining symbolism and connectionism.
The discrete structure given by a sharp distribution can be considered as the computation graph in symbolic system.
The sharpness of the distribution can guarantee that information can only combined or communicated through the induced structure.
In a tree-like structure, this effect can create information bottlenecks.
So the model can learn the vector representation of a phrase or a sentence.
This is similar to symbolic system, that we can find many intermediate results in the computation graph, before getting the final result.
These intermediate results contributes to the excellent interpretability of symbolic methods.
Similarly, for Ordered Memory model, we can also find these intermediate result stored in memory slots.
For example, after processing a ListOps equation, each memory slot represent the value of a parenthesis in the equation.

In our work, we proposed ON-LSTM and UDGN to learn different type of latent structures.
However, how to emerge sharp distributions and get interpretable intermediate results in a natural language task still remains a open question to study.

\section{Inducing Reusable Operators}
Once a model could stably produce discrete structure, a reasonable next step is trying to replace the single composition/communicate function by a set of operators.
For example, in UDGN, we use the competitive mechanism to select different communication channels for each pair of tokens.
In OCN, we have different options for different subtasks.
The idea is inspired by the operators in the formal language and the syntactic functions in theoritical linguistics.
In Logical Inference, we have operators like \textit{or} and \textit{and}.
In dependency grammar, we have syntactic functions like \textit{SUBJ} and \textit{PRED}.
One common feature of these operators are the resusability.
It means that the same operator can be used in many different contexts and still hold the same functionality.
The only constraint is that inputs of the operator should share some common features.

Introducing a set of operators have two major advantages.
The first one is reducing the complexity of model components.
For example, in ListOps, if the composition function needs model \texttt{MAX}, \texttt{SUM} and \texttt{MEAN} at the same time, it should require more capacity then modeling only one operation.
Secondly, simpler operator usually have a better reusability, because they require less input information and is less sensitive to the context.
For example, in OCN, an option that models only one subtask can be reused by any controller when the subtask is encountered.
If the option models two different subtasks, the controller will have to pass a command vector to the option to disambiguate the subtask.
This command vector could cause extra effort for the new controller to learn the protocol.

In our work, UDGN provide a potential solution to learn syntactic functions in natural language setting. 
In a undirected dependency graph, UDGN uses a competitive mechanism to select module for each edge to propagate information.
But, how to clearly define an learn reusable operators in natural language tasks still remains a open question.

\section{Systematic Generalization}
In a symbolic framework, systematic generalization is straightforward.
Once the operators and grammar are well-defined, any inputs that satisfy the pre-defined grammar can be process by the system.
However, this setting also have great limitations in real world.
Firstly, natural language has very complicate grammar, that even a state of the art parser could fail in many cases.
Secondly, the operators used by natural language are complicated and difficult to be pre-defined.
In this thesis, we try to solve the two problem with a date-driven approach, that is given a pre-designed inductive bias, we want the model to induce the syntax and operators from the supervised or unsupervised training losses.
We observe some successes on synthetic tasks, including ListOps, Logical Inference and Craft. 
But reaching systematic generalization on natural language still require a lot of effort and creativity. 

